A Statistical Investigation of Long Memory in Language and Music

Representation and learning of long-range dependencies is a central challenge confronted in modern applications of machine learning to sequence data. Yet despite the prominence of this issue, the basic problem of measuring long-range dependence, either in a given data source or as represented in a trained deep model, remains largely limited to heuristic tools. We contribute a statistical framework for investigating long-range dependence in current applications of deep sequence modeling, drawing on the well-developed theory of long memory stochastic processes. This framework yields testable implications concerning the relationship between long memory in real-world data and its learned representation in a deep learning architecture, which are explored through a semiparametric framework adapted to the high-dimensional setting.

==> sections/simulations.tex <==
In this section we provide plots of the objective function computed over a fine grid of $d$ values on both simulated and real data. The visualizations for real data also include plots of the periodogram near the origin, and an exploration of the potential bias in the Gaussian semiparametric estimator using the King James Bible data.

\subsection{Simulated data}

We generate sequences of length $N = 2^{14} = 16384$ from two models of scalar long memory processes: fractionally differenced Gaussian white noise (FD) and an order-3 stationary ARFIMA model. Sample sequences are drawn for values of $d$ ranging from $-0.4$ to $0.4$ in increments of $0.1$. We plot the objective that is minimized in the estimation of $d$ as a function of $d$ for the FD and ARFIMA data in Figures \ref{fig:fd_sim} and \ref{fig:arfima_sim}, respectively.

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/fracdiff_sim.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for realizations of a fractionally differenced process over a range of true $d$ values. The title of each plot indicates the true value of $d$ and the estimated $\hat{d}$ resulting from minimization of $R(d)$.}
\label{fig:fd_sim}
\end{figure}

\begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/arfima_sim.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for realizations of an ARFIMA process over a range of true $d$ values. The title of each plot indicates the true value of $d$ and the estimated $\hat{d}$ resulting from minimization of $R(d)$.}
\label{fig:arfima_sim}
\end{figure}
\newpage

\subsection{Real data}

\subsubsection{Recurrent models}

In this section we plot the objective function against $d$ for the scalar process corresponding to the first hidden node of our four recurrent models. We also include plots of the log periodogram against negative log Fourier frequences near the origin; geometrically, the long memory parameter $d$ is the slope of this curve as $\lambda_j \to 0$.

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/recurrent_viz_1d.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for the first hidden node in each of our recurrent models.}
\label{fig:rviz1}
\end{figure}

We also include two-dimensional plots of the objective for the process defined by the first two hidden nodes of the recurrent models. As in the one-dimensional case, the minimum appears to be achieved close to the origin.

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/recurrent_viz_2d.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for first two hidden nodes in each of our recurrent models.}
\label{fig:rviz2}
\end{figure}

\newpage

\subsubsection{Bach fugues}

We include the same plots as above for the scalar process corresponding to the first hidden node of the embedded Bach fugues. While the information represented is the same, in this case we note that the estimated long memory parameters are significantly away from zero, which is confirmed by the positive slope in the log-periodogram plots.

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/bach_viz.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for the first hidden dimension of the embedded Bach fugues.}
\label{fig:bach_viz}
\end{figure}

\newpage

\subsubsection{Bible text}

Finally, we include a plot of the objective and log-periodogram for the first hidden node of the embedded Bible text. Again, the result shows that the minimum (and therefore the estimated long memory parameter) is positive.

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/bible_viz.pdf}
\caption{\small Objective $R(d)$ vs. $d$ for the first hidden dimension of the embedded Bible text.}
\label{fig:bible_viz}
\end{figure}

Finally, we include a comparison study that shows the potentially significant effect of bias in semiparametric estimation of long memory. In Figure \ref{fig:bible_bias}, we show the log-periodogram plot over a range of periodogram window sizes. A larger window corresponds to denser estimation of the periodogram. For each window size $N$, the bandwidth of the Gaussian semiparametric estimator is set to be $m = \sqrt{N}$. This corresponds to a cutoff indicated by the vertical red line; only periodogram ordinates to the right of this line are used to estimate the long memory. As shown by the estimated $\hat{d}$ for each choice of $N$, this can have a significant impact on the result. The impact depends on the shape of the periodogram, which for real-world data is not known a priori. Essentially, bias is introduced when the bandwidth is large enough to capture parts of the periodogram that do not represent local behavior around the origin. We conclude that it is safest to take conservative choices of $m$, and that results should only be trusted if the periodogram can be estimated relatively densely around the origin.  

 \begin{figure}[h!]
\centering 
\includegraphics[width=.95\textwidth]{../../figures/bible_bias.pdf}
\caption{\small Log periodogram of embedded Bible process for window size $N$ and bandwidth parameter $m = \sqrt{N}$. Red line indicates the bandwidth cutoff for estimation of long memory. Note that despite the fact that $m$ increases with $N$, the bandwidth for estimation around the origin decreases at $N$ grows.}
\label{fig:bible_bias}
\end{figure}



